Domain Generalization Guided by Gradient Signal to Noise Ratio of Parameters

Overfitting to the source domain is a common issue in gradient-based training of deep neural networks. To compensate for the over-parameterized models, numerous regularization techniques have been introduced such as those based on dropout. While these methods achieve significant improvements on classical benchmarks such as ImageNet, their performance diminishes with the introduction of domain shift in the test set i.e. when the unseen data comes from a significantly different distribution. In this paper, we move away from the classical approach of Bernoulli sampled dropout mask construction and propose to base the selection on gradient-signal-to-noise ratio (GSNR) of network's parameters. Specifically, at each training step, parameters with high GSNR will be discarded. Furthermore, we alleviate the burden of manually searching for the optimal dropout ratio by leveraging a meta-learning approach. We evaluate our method on standard domain generalization benchmarks and achieve competitive results on classification and face anti-spoofing problems.

==> _constants.tex <==
\def\cvprPaperID{10787}
\def\confName{ICCV}
\def\confYear{2023}

\def\paperTitle{Domain Generalization Guided by Gradient Signal to Noise Ratio of Parameters}

\def\authorBlock{
    Author 1\thanks{Equal contribution} \qquad
    Author 2\footnotemark[1] \qquad
    Author 3 \\
    Institute \\
    {\tt\small \{email, addresses\}@inst.edu}
}

% Compilation vars
\newif\ifreview \newcommand{\review}{\reviewtrue}
\newif\ifarxiv \newcommand{\arxiv}{\arxivtrue}
\newif\ifcamera \newcommand{\cameraready}{\cameratrue}
\newif\ifrebuttal \newcommand{\rebuttal}{\rebuttaltrue}


==> cvpr_header.tex <==
\ifreview \usepackage[review]{cvpr} \fi
\ifarxiv \usepackage[pagenumbers]{cvpr} \fi
\ifrebuttal \usepackage[rebuttal]{cvpr} \fi
\ifcamera \usepackage{cvpr} \fi

\usepackage{graphicx}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{booktabs}

\usepackage{xcolor}

\input{_macros}  % Add packages to _macros.tex

%% For cross-referencing labels between documents
\usepackage{xr-hyper}

\makeatletter
\newcommand*{\addFileDependency}[1]{
  \typeout{(#1)}
  \@addtofilelist{#1}
  \IfFileExists{#1}{}{\typeout{No file #1.}}
}

\makeatother
\newcommand*{\myexternaldocument}[1]{
    \externaldocument{#1}
    \addFileDependency{#1.tex}
    \addFileDependency{#1.aux}
}
%%

\usepackage[pagebackref,breaklinks,colorlinks]{hyperref}
\usepackage[capitalize]{cleveref}
\crefname{section}{Sec.}{Secs.}
\crefname{table}{Table}{Tables}
\crefname{figure}{Fig.}{Figs.}

\frenchspacing


==> figs/cam_gsnr.tex <==
\begin{figure}
    \centering
     \includegraphics[width=0.6\linewidth]{figs/arxiv_cam_gsnr.pdf}
    \caption{Localization of domain-specific regions through Class Activation Mappings}
    \label{fig:cam}
\end{figure}

==> figs/p_over_time.tex <==
\begin{figure}
    \centering
     \includegraphics[width=\linewidth]{figs/p_over_time.pdf}
    \caption{Evolution of dropout ratio over time for our grid-based approach and meta-based approach.}
    \label{fig:p_over_time}
\end{figure}


==> figs/rsc_vs_ours.tex <==
\begin{figure}
    \centering
     \includegraphics[width=\linewidth]{figs/rsc_issues.pdf}
     % \vspace{-2ex}
    \caption{\revision{Different approaches to dropout mask construction: RSC and ours. Our approach replaces random seeds with those based on the gradients and follows a standard placement and scheduler mechanisms (marked in purple). RSC introduces a number of hyperparameters (marked in red) when constructing placement algorithm and scheduler.
    Additionally, dropout ratios for each ResNet block are chosen manually for RSC (marked in light blue) while in our approach those parameters are learned (marked in green)}}
    \label{fig:rsc_vs_ours}
    % \vspace{-2ex}
\end{figure}

==> figs/ssan_ours.tex <==
\begin{figure}
    \centering
     \includegraphics[width=\linewidth]{figs/arxiv_ssan_ours.pdf}
     \vspace{-2ex}
    \caption{Depiction of the face anti-spoofing method SSAN \cite{wang2022domain} equipped with our GSNR-guided dropout technique.}
    \label{fig:ssan_ours}
    \vspace{-2ex}
\end{figure}

==> list_sup/forward_pass.tex <==
\begin{figure*}[t]
\begin{lstlisting}[caption={Forward pass example.},captionpos=b]
# forward pass to obtain gradients
class_logit, ResNetBlocks = model(images, labels, grads=None)
loss = criterion(class_logit, labels)
grads = [ torch.autograd.grad(loss, ResNetBlock)[0] for ResNetBlock in ResNetBlocks]
# forward pass to apply GSNR-guided GSNR
class_logit, _ = task_model(data, labels, grads)
loss = criterion(class_logit, labels)
loss.backward()
optimizer.step() 
\end{lstlisting}
\end{figure*}

==> tables/ablation_m1_m2.tex <==
\begin{table}
\centering
\captionof{table}{\revision{Ablation study: impact of the intermediate masks 
on the proposed \textit{Meta-GSNR} approach. For simplicity, we denote $0$ and $1$ as all-zeros and all-ones matrices.}} 
\scalebox{0.67}{
\begin{tabular}{ |c|c|c|c|c|c| } 
 \hline
 PACS                                & artpaint & cartoon  & sketch  & photo    & Avg $\uparrow$  \\ \hline
 Meta-GSNR w/$M^{(1)} \cdot M^{(2)}=0$         &10.88     & 21.84    & 04.42     & 16.64   & 13.44  \\
 Meta-GSNR w/$M^{(1)}=1$         & 78.12    &  76.57  & 75.16   & 94.49 & 81.08 \\
 Meta-GSNR w/($M^{(2)}=1$         &80.85   & 80.73    & 81.85   & 94.79 & 84.55    \\
 Meta-GSNR w/$M^{(1)}=M^{(2)}=1$         & 77.49    & 77.21   & 72.67  & 92.45 & 79.95  \\
 \hline
 Meta-GSNR                 & 83.64    & 80.03    & 84.37     & 95.32   & \textbf{85.84}  \\
 \hline
\end{tabular} }
\label{table.ablation_m1_m2}
\end{table}


==> tables/architectures.tex <==
\begin{table}[!h]
% \vspace{-2ex}
\centering\small
\captionof{table}{\revision{Classification accuracy (\%) on PACS~\cite{li2017deeper} using various backbones. The bold numbers indicate the best performance averaged across all test domains.}}
% \vspace{-2ex}
\scalebox{0.84}{
\begin{tabular}{ |c|c|c|c|c|c|c| } 
 \hline
 \multicolumn{2}{|c|}{PACS}                                & artpaint & cartoon  & sketch  & photo    & Avg $\uparrow$  \\ \hline
  \multirow{4}{*}{\rotatebox{90}{\centering AlexNet }} 
 & MASF~\cite{dou2019domain}  & 70.35 & 72.46 & 67.33 & 90.68 &  75.21      \\
 & DMG~\cite{chattopadhyay2020learning}& 64.65 & 69.88 & 71.42 & 87.31 &  73.32        \\
 & RSC~\cite{huang2020self}   & 70.93 & 71.62 & 71.35 & 90.23 & 76.03                \\ 
 & Ours                       & 72.25 & 73.23 & 70.69 & 91.52 & \textbf{76.92}                 \\
 \hline
  \multirow{4}{*}{\rotatebox{90}{\centering ResNet18 }} 
 & MASF~\cite{dou2019domain}  & 80.29   & 77.17 & 71.68 & 94.99 & 81.03 \\
 & DMG~\cite{chattopadhyay2020learning}& 76.90 & 80.38 & 75.21 & 93.35 &  81.46 \\
 & RSC~\cite{huang2020self}   &   80.73 & 79.22 & 81.48 & 94.16  & 83.90    \\ 
 & Ours                                & 83.64    & 80.03    & 84.37     & 95.32   & \textbf{85.84}  \\
 \hline
   \multirow{4}{*}{\rotatebox{90}{\centering ResNet50 }} 
 & MASF~\cite{dou2019domain}  & 82.89 & 80.49 & 72.29 & 95.01 &  82.67      \\
 & DMG~\cite{chattopadhyay2020learning}& 82.57 & 78.11 & 78.32 & 94.49 &  83.37        \\
 & ITL-Net~\cite{gao2022loss} & 87.1 &83.3 &96.1 & 79.3& 86.4\\
 & EoA~\cite{arpit2022ensemble} &90.5 & 83.4&98.0 &82.5 &88.6\\
 & DNA~\cite{chu2022dna} &89.8 &83.4 &97.7 &82.6 &88.4\\
 & Style Neophile~\cite{kang2022style} &90.35 &84.20 &96.73 &85.18 &89.11\\
 & RSC~\cite{huang2020self}   & 84.08 & 84.59 & 83.76 & 95.56 & 86.99          \\ 
 & Ours                       & 87.93 & 85.53 & 86.68 & 96.83  & \textbf{89.24}                \\
 \hline
\end{tabular}}
\label{tab:pacs_archs}
\end{table}

==> tables/digits-dg.tex <==
\begin{table}[h]

\centering  %\small
% \scriptsize{
\captionof{table}{\revision{Classification accuracy (\%) on the Digits-DG dataset~\cite{zhou2020learning}. The bold numbers indicate the best performance averaged across all test domains.}}
\label{tab:digits_dg}
\scalebox{0.74}{
\begin{tabular}{ |c|c|c|c|c|c|c| } 
 \hline
Digits-DG & MNIST & MNIST-M & USPS & SVHN & Synthetic & Avg $\uparrow$ \\\hline
% \\ 
% \hline
  Baseline & 86.15 & 74.44 & 90.07 & 81.29 & 94.46 & 85.28 \\
 DSBN~\cite{chang2019domain} & 87.01 & 71.20 & 91.18 & 78.23 & 94.30 & 84.38 \\
 SN~\cite{luo2018differentiable} & 89.28 & 78.40 & 88.54 & 79.12 & 95.66 & 86.20 \\
DSON~\cite{seo2020learning} & 89.62 & 79.00 & 91.63 & 81.02 & 95.34 & 87.32 \\
Ours & 96.97 & 84.38 & 90.82 &  80.11& 96.21 & \textbf{89.69}   \\   
 \hline
 
\end{tabular}}
\end{table}


==> tables/ocim.tex <==
\begin{table*}[!h]
\centering

 \captionof{table}{Classification accuracy (\%) on the OCIM dataset. The bold numbers indicate the best performance in each setting. For more results we refer to the supplementary material} 
\small
\begin{tabular}{ |c|c|c|c|c|c|c|c|c| } 

 
 \hline
\multicolumn{1}{|c|}{\multirow{1}[4]{*}{Method}} & \multicolumn{2}{c|}{O\&C\&I to M} & \multicolumn{2}{c|}{O\&M\&I to C} & \multicolumn{2}{c|}{O\&C\&M to I} & \multicolumn{2}{c|}{I\&C\&M to O} \\
\cline{2-9}          & \multicolumn{1}{l|}{HTER(\%) $\downarrow$}  & \multicolumn{1}{c|}{AUC(\%) $\uparrow$} & \multicolumn{1}{l|}{HTER(\%)$\downarrow$} & \multicolumn{1}{c|}{AUC(\%) $\uparrow$} & \multicolumn{1}{l|}{HTER(\%)$\downarrow$} & \multicolumn{1}{c|}{AUC(\%) $\uparrow$} & \multicolumn{1}{l|}{HTER(\%)$\downarrow$} & \multicolumn{1}{c|}{AUC(\%) $\uparrow$} \\ \hline
 MMD-AAE \cite{li2018domain}              & 27.08    & 83.19    & 44.59    & 58.29   & 31.58    &  75.18  & 40.98    & 63.08           \\
MADDG~\cite{shao2019multi}                 & 17.69    & 88.06   & 24.50    & 84.51   & 22.19    & 84.99   & 27.98    & 80.02      \\
DR-MD-Net~\cite{wang2020cross}             & 17.02    & 90.10   & 19.68    & 87.43   & 20.87    & 86.72   & 25.02    & 81.47        \\
RFMeta~\cite{shao2020regularized}                & 13.89    & 93.98   & 20.27    & 88.16   & 17.30    & 90.48   & 16.45    & 91.16      \\
NAS-FAS~\cite{yu2020fas}               & 19.53    & 88.63   & 16.54    & 90.18   & 14.51    & 93.84   & 13.80    & 93.43        \\
D2AM~\cite{chen2021generalizable}                  & 12.70    & 95.66   & 20.98    & 85.58   & 15.43    & 91.22   & 15.27    & 90.87        \\
SDA~\cite{wang2021self}                  & 15.40    & 91.80   & 24.50    & 84.40   & 15.60    & 90.10   & 23.10    & 84.30         \\
DRDG~\cite{liudual}                  & 12.43    & 95.81   & 19.05    & 88.79   & 15.56    & 91.79   & 15.63    & 91.75     \\
ANRL~\cite{liu2021adaptive}                  & 10.83    & 96.75   & 17.83    & 89.26   & 16.03    & 91.04   & 15.67    & 91.90         \\
SSAN                       & 2.50   & 97.50 & 13.59 &93.67  & 17.62 & 83.91 & 19.15 & 87.95 \\
 SSAN + Ours               & 2.50   & 95.50 & 10.94 &95.17  & 12.25 & 93.60 & 18.42 &  88.63 \\
 \hline
 \end{tabular}
 \label{table.ocim}
\end{table*}

 








 




 




==> tables/ocim_hter.tex <==
\begin{table*}[h]
\centering

 \captionof{table}{Classification accuracy (\%) on the OCIM dataset. The bold numbers indicate the best performance in each setting. For more results, refer to the supplementary material.} 
\scalebox{0.8}{
\begin{tabular}{ |c|c|c|c|c|c|c|c|c|c| } 

 
 \hline
\multicolumn{1}{|c|}{\multirow{1}[4]{*}{Method}} & \multicolumn{2}{c|}{O\&C\&I to M} & \multicolumn{2}{c|}{O\&M\&I to C} & \multicolumn{2}{c|}{O\&C\&M to I} & \multicolumn{2}{c|}{I\&C\&M to O} & Avg HTER \\
\cline{2-9}          & \multicolumn{1}{l|}{HTER(\%) $\downarrow$}  & \multicolumn{1}{c|}{AUC(\%) $\uparrow$} & \multicolumn{1}{l|}{HTER(\%)$\downarrow$} & \multicolumn{1}{c|}{AUC(\%) $\uparrow$} & \multicolumn{1}{l|}{HTER(\%)$\downarrow$} & \multicolumn{1}{c|}{AUC(\%) $\uparrow$} & \multicolumn{1}{l|}{HTER(\%)$\downarrow$} & \multicolumn{1}{c|}{AUC(\%) $\uparrow$} &  \\ \hline
 MMD-AAE \cite{li2018domain}              & 27.08    & 83.19    & 44.59    & 58.29   & 31.58    &  75.18  & 40.98    & 63.08  &  36.05        \\
MADDG~\cite{shao2019multi}                 & 17.69    & 88.06   & 24.50    & 84.51   & 22.19    & 84.99   & 27.98    & 80.02  &  23.09    \\
DR-MD-Net~\cite{wang2020cross}             & 17.02    & 90.10   & 19.68    & 87.43   & 20.87    & 86.72   & 25.02    & 81.47  &  20.64      \\
RFMeta~\cite{shao2020regularized}                & 13.89    & 93.98   & 20.27    & 88.16   & 17.30    & 90.48   & 16.45    & 91.16 & 16.97    \\
D2AM~\cite{chen2021generalizable}                  & 12.70    & 95.66   & 20.98    & 85.58   & 15.43    & 91.22   & 15.27    & 90.87  & 16.09      \\
SDA~\cite{wang2021self}                  & 15.40    & 91.80   & 24.50    & 84.40   & 15.60    & 90.10   & 23.10    & 84.30  &  19.65     \\
DRDG~\cite{liudual}                  & 12.43    & 95.81   & 19.05    & 88.79   & 15.56    & 91.79   & 15.63    & 91.75  &  15.66  \\
ANRL~\cite{liu2021adaptive}                  & 10.83    & 96.75   & 17.83    & 89.26   & 16.03    & 91.04   & 15.67    & 91.90  & 15.09      \\ 
  
\hline
SSAN                       & 2.50   & 97.50 & 13.59 &93.67  & 17.62 & 83.91 & 19.15 & 87.95  & 13.21\\
 SSAN + Ours               & 2.50   & 95.50 & 10.94 &95.17  & 12.25 & 93.60 & 18.42 &  88.63 & 11.02 \\
 EPCR\cite{wang2023consistency}  & 11.36 & 91.98 \\
 EPCR + ours & \textbf{10.47} & \textbf{93.28}  \\
 \hline
 \end{tabular}}
 \label{table.ocim_hter}
\end{table*}




 








 




 




==> tables/vlcs.tex <==
\begin{table}[h]

\centering  %\small
% \scriptsize{
\vspace{-1ex}
\captionof{table}{\revision{Classification accuracy (\%) on the VLCS dataset~\cite{torralba2011unbiased}. The bold numbers indicate the best performance averaged across all test domains.}}
\label{tab:vlcs}
\scalebox{0.85}{
\begin{tabular}{ |c|c|c|c|c|c| } 
 \hline
VLCS & Caltech & LabelMe & VOC2007 & SUN09 & Avg $\uparrow$ \\\hline
% \\ 
% \hline
  Baseline   & 96.25 & 59.72 & 70.58 & 64.51  & 72.76  \\
  JiGen~\cite{carlucci2019domain} & 96.93 & 60.90 & 70.62 & 64.30  & 73.19 \\
  RSC~\cite{huang2020self}   & 97.61 & 61.86 & 73.93 & 68.32  & 75.43 \\
Ours &97.49   & 65.47   & 73.82  & 68.43  & \textbf{76.30}    \\
 \hline
 
\end{tabular}}
\end{table}


==> tables_sup/pacs_sup.tex <==
\begin{table}[!h]
\centering\small
\captionof{table}{Classification accuracy (\%) on the PACS dataset \cite{li2017deeper}. The bold numbers indicate the best performance in each setting.}
\begin{tabular}{ |c|c|c|c|c|c| } 
 \hline
 PACS                                & artpaint & cartoon  & sketch  & photo    & Avg $\uparrow$  \\ \hline
\multicolumn{6}{|c|}{Pre-trained on ImageNet} \\ \hline
  Baseline                           & 78.63    & 75.27    & 68.72   & 96.08    &79.68  \\

 RSC   \cite{huang2020self}                        &   80.73 & 79.22 & 81.48 & 94.16  & 83.90    \\ 
 
 Ours                                & 83.64    & 80.03    & 84.37     & 95.32   & \textbf{85.84}  \\
 \hline
 \multicolumn{6}{|c|}{Trained from scratch} \\ \hline
 Baseline                           &   52.19  & 65.01 & 68.23 & 75.38  & 65.20      \\
 
 RSC   \cite{huang2020self}      & 56.49& 65.74 & 80.05&  68.64&67.72 \\
 Ours               &  60.55& 69.50  &  72.74 & 78.14&  \textbf{70.23}\\ \hline


\end{tabular}
\label{tab:pacs_sup}
\end{table}
